Combining the Best of Graphical Models and ConvNets for Semantic Segmentation

We present a two-module approach to semantic segmentation that incorporates Convolutional Networks (CNNs) and Graphical Models. Graphical models are used to generate a small (5-30) set of diverse segmentations proposals, such that this set has high recall. Since the number of required proposals is so low, we can extract fairly complex features to rank them. Our complex feature of choice is a novel CNN called SegNet, which directly outputs a (coarse) semantic segmentation. Importantly, SegNet is specifically trained to optimize the corpus-level PASCAL IOU loss function. To the best of our knowledge, this is the first CNN specifically designed for semantic segmentation. This two-module approach achieves $52.5\%$ on the PASCAL 2012 segmentation challenge.

==> figs/fig1.tex <==
\begin{figure}
    \begin{center}
        \begin{subfigure}[c]{\columnwidth}
            \begin{overpic}[width=\columnwidth]{figs/bird_conv.png}
            \end{overpic}
            \caption{}
            \label{fig:conv_a}
        \end{subfigure}
        \begin{subfigure}[c]{\columnwidth}
        \begin{overpic}[width=\columnwidth]{figs/fig1_img.png}
            \put(82, 14){\color{white}\scriptsize airplane}
        \end{overpic}
            \caption{}
            \label{fig:conv_b}
        \end{subfigure}
    \end{center}
\vspace{-2em}
    \caption{We predict a coarse image labeling directly from our Convolutional
    Neural Network (CNN). In \ref{fig:conv_a} a map of first layer activations is
    visualized. The rectangles with ?s are filters which are learned by the CNN.
    Figure \ref{fig:conv_b} shows that multiple feature maps are produced and
    combined in layers to finally produce a soft segmentation output. This
    architecture isn't the one we used, but simply meant to convey intuition.}
\vspace{-1em}
\end{figure}



==> figs/fig2.tex <==
\begin{figure*}
    \begin{minipage}[c]{0.14\textwidth}
    \begin{subfigure}[c]{\textwidth}
        \includegraphics[width=\textwidth]{figs/bird_img}
        \begin{overpic}[width=\textwidth]{figs/bird_argmax}
            \put(47, 38){\color{white}\scriptsize bird}
        \end{overpic}
        \caption{}
        \label{fig:argmax}
    \end{subfigure}
    \end{minipage}
    \
    \begin{minipage}[c]{0.5\textwidth}
    \begin{subfigure}[c]{\textwidth}
        \includegraphics[width=\textwidth]{figs/bird_21}
        \caption{}
        \label{fig:chan}
    \end{subfigure}
    \end{minipage}
    \
    \begin{minipage}[c]{0.35\textwidth}
    \begin{subfigure}[c]{\textwidth}
        \hspace{1.5em}
        \begin{minipage}[c]{0.23\textwidth}
            \begin{overpic}[width=\textwidth]{figs/bird_original_0}
                \put(27, 23){\color{white}\scriptsize bird}
            \end{overpic}
            \begin{overpic}[width=\textwidth]{figs/bird_original_1}
                \put(27, 23){\color{white}\scriptsize bird}
            \end{overpic}
            \begin{overpic}[width=\textwidth]{figs/bird_original_2}
                \put(27, 23){\color{white}\scriptsize bird}
            \end{overpic}
            \makebox[\textwidth]{\vdots}
        \end{minipage}
        \hfill
        \setlength{\unitlength}{1em}
        \begin{minipage}[c]{0.3\textwidth}
            \begin{picture}(0, 0)
                \put(0, 1){\vector(3,2){5}}
                \put(0, 5){\vector(1,-2){5}}
                \put(0, -3){\vector(3,-0){5}}
                \put(0, -6){\vector(2,3){5}}
            \end{picture}
        \end{minipage}
        \hfill
        \begin{minipage}[c]{0.23\textwidth}
            \begin{overpic}[width=\textwidth]{figs/bird_rerank_0}
                \put(27, 23){\color{white}\scriptsize bird}
            \end{overpic}
            \begin{overpic}[width=\textwidth]{figs/bird_rerank_1}
                \put(27, 23){\color{white}\scriptsize bird}
                \put(45, 60){\color{white}\scriptsize plant}
            \end{overpic}
            \begin{overpic}[width=\textwidth]{figs/bird_rerank_2}
                \put(27, 23){\color{white}\scriptsize bird}
            \end{overpic}
            \makebox[\textwidth]{\vdots}
        \end{minipage}
        \hspace{1.5em}
        \caption{}
        \label{fig:rank}
    \end{subfigure}
    \end{minipage}
    \begin{subfigure}{\textwidth}
        \caption*{
        ~\ref{fig:argmax} An Image and corresponding Coarse Segmentation
        produced by our CNN. The bottom image is the pixel-wise argmax over
        classes of the net's output.
        ~\ref{fig:chan} A class-wise breakdown of predictions by our CNN. This,
        as opposed to the argmax in ~\ref{fig:argmax} is what the net actually
        produces.
        ~\ref{fig:rank} The top 3 of 10 O$_{2}$P+DivMBest segmentations before
        (left) and after (right) re-ranking by similarity to coarse segmentations.
        The CNN correctly selects the slender bird segmentation, but ranks
        a similar segmentation where DivMBest also thinks a plant is present second.
        }
    \end{subfigure}
    \caption{Examples}
    \label{fig:examples}
\end{figure*}
\begin{table*}
\scriptsize
\begin{tabu} to \linewidth {lX[c]X[c]X[c]X[c]X[c]X[c]X[c]X[c]X[c]X[c]X[c]X[c]X[c]X[c]X[c]X[c]X[c]X[c]X[c]X[c]X[c]|X[c]}
& \begin{turn}{90}Backgr.\end{turn} &  \begin{turn}{90}Plane\end{turn} &  \begin{turn}{90}Bicycle\end{turn} &  \begin{turn}{90}Bird\end{turn} &  \begin{turn}{90}Boat\end{turn} &  \begin{turn}{90}Bottle\end{turn} &  \begin{turn}{90}Bus\end{turn} &  \begin{turn}{90}Car\end{turn} &  \begin{turn}{90}Cat\end{turn} &  \begin{turn}{90}Chair\end{turn} &  \begin{turn}{90}Cow\end{turn} &  \begin{turn}{90}D.Table\end{turn} &  \begin{turn}{90}Dog\end{turn} &  \begin{turn}{90}Horse\end{turn} &  \begin{turn}{90}M.bike\end{turn} &  \begin{turn}{90}Person\end{turn} &  \begin{turn}{90}Plant\end{turn} &  \begin{turn}{90}Sheep\end{turn} &  \begin{turn}{90}Sofa\end{turn} &  \begin{turn}{90}Train\end{turn} &  \begin{turn}{90}TV.Mon\end{turn} &  \begin{turn}{90}Average\end{turn} \\
\hline
O$_{2}$P ~\cite{carreira_eccv12} &
         84.8 & 63.7 & 23.4 & 44.9 & 40.8 & 45.1 & 58.0 & 58.8 & 57.6 & 12.1 & 43.8 & 31.0 & 44.8 & 56.2 & 56.8 & 52.3 & 37.1 & 44.0 & 29.5 & 48.6 & 42.9 & 46.5 \\
O$_{2}$P DivMBest+ReRank ~\cite{yadollahpour2013rerank} &
         85.7 & 62.7 & 25.6 & 46.9 & 43.0 & 54.8 & 58.4 & 58.6 & 55.6 & 14.6 & 47.5 & 31.2 & 44.7 & 51.0 & 60.9 & 53.5 & 36.6 & 50.9 & 30.1 & 50.2 & 46.8 & 48.1 \\
%Ours (CVPR workshop)   & 85.1 & \textbf{69.5} & \textbf{25.8} & \textbf{59.9} & \textbf{44.0} & 33.3 & \textbf{69.0} &58.0&56.8& \textbf{15.1} & 41.2 & 20.2 & \textbf{51.1} & 41.6 & 52.4 & \textbf{54.3} & 34.4 & \textbf{61.3} & 22.9 & \textbf{59.8} & 40.3 & 47.4 \\
SDS ~\cite{hariharan2014sds} & \textbf{86.7} & 63.3 & 25.7 & \textbf{63.0} & 39.8 & \textbf{59.2} & \textbf{70.9} & \textbf{61.4} & 54.9 & \textbf{16.8} & 45.0 & \textbf{48.2} & 50.5 & 51.0 & 57.7 & \textbf{63.3} & 31.8 & 58.7 & 31.2 & \textbf{55.7} & \textbf{48.5} & 51.6 \\
Segnets & 86.6 & \textbf{65.3} & \textbf{27.4} & 57.7 & \textbf{44.5} & 57.1 & 68.6 & 60.9 & \textbf{57.8} & 14.5 & \textbf{59.6} & 33.3 & \textbf{51.6} & \textbf{56.6} & \textbf{64.1} & 59.2 & \textbf{38.9} & \textbf{62.4} & \textbf{34.0} & 48.9 & 47.3 &  \textbf{52.2} \\
\hline
\end{tabu}
\caption{
TODO: fill in the rest of the table once the evaluation server comes back online  
PASCAL VOC 2012 segmentation results. ~\cite{carreira_eccv12} is the same as picking the highest scoring DivMBest solution.}
\label{tab:results}
\end{table*}


==> figs/fig3.tex <==
\begin{figure*}

\includegraphics[width=\textwidth]{figs/segnet_ppt.pdf}
\vspace{-2em}
    \caption{We predict a coarse image labeling directly from our Convolutional
    Neural Network. By combining this segmentation with other features,
    we can learn to rank a diverse set of whole-image segmentation proposals.}
\vspace{-1em}
\end{figure*}


==> objective.tex <==
	The standard evaluation criteria used in segmentation tasks is the average Intersection-over-Union(IOU) across classes which is defined as:
\begin{gather}
IOU = \frac{1}{K}\sum_k IOU_k \\
= \frac{1}{K}\sum_k\frac{TP_k}{TP_k+FP_k+FN_k}\\
= \frac{1}{K}\sum_k\frac{GT_k-FN_k}{GT_k+FP_k}
\end{gather}

Often the challenging task with learning based methods is to pick an objective function which is suitable for optimisation and also shares a correlation to the actual evaluation metric. An ideal loss function is expected to have a gradient whose magnitude is proportional to the number of false labels. In the case of segmentation tasks, it might seem intuitive to optimise over a objective gain function equal to the Intersection-over-Union. Here we show that the IOU function inherently has a certain bias which makes its performance as an objective function far from ideal. We then show that Union-over-Intersection(UOI) acts as a better objective function and also explain that minimising UOI leads to maximisation of IOU. 

\paragraph{Intersection-over-Union}
Consider the following gradient of the $IOU_k$ gain function for class $k$ with respect to the false labels $FP_k$ and $FN_k$:
\begin{gather} \frac{\partial (IOU_k)}{\partial (FP_k)} = \frac{-(GT_k-FN_k)}{(GT_k+FP_k)^2}\\
\frac{\partial (IOU_k)}{\partial (FN_k)} = \frac{-1}{GT_k+FP_k}
\end{gather}
Clearly,\\
	$$ \frac{\partial (IOU_k)}{\partial (FP_k)}\to 0 \hspace{5pt}   for\hspace{5pt} FP_k>> 0, \hspace{5pt} and,$$
	$$ \frac{\partial (IOU_k)}{\partial (FN_k)}\to 0 \hspace{5pt}   for\hspace{5pt} FP_k>> 0, \hspace{5pt} and,$$
These properties of the IOU function are not desirable in an objective function:\\
1) For large number of wrong labels, the gradient is zero. This would have the affect of not penalising over-prediction of classes and is more predominant in classes which have large ground truths.\\
2) For the case where all pixels are mislabeled, $FN_k=GT_k$ and $FP_k>>0$, all gradients are very small.\\

The implications are that more importance is given to larger classes(in most cases, the background class) since the upper bound on $FP_k$ is smaller. This could lead to prediction of the whole image as background unless the parameters are initialised with great care.\\

\paragraph{Union-over-Intersection}


Now we show that Union-over-Intersection(UOI) infact acts as a better optimisation function due to the behaviour of its gradient and also that it shares a seemingly obvious relation with the IOU function. The $UOI$ function can be written as:
\begin{gather}
UOI = \frac{1}{K}\sum_k UOI_k\\
= \frac{1}{K}\sum\frac{TP_k + FP_k + FN_k}{TP_k}\\
= \frac{1}{K}\sum_k\frac{GT_k+FP_k}{GT_k-FN_k}
\end{gather}

Consider the gradient of the $UOI_k$ function w.r.t the false labels $FP_k$ and $FN_k$:
\begin{gather}
\frac{\partial UOI_k}{\partial FP_k} = \frac{1}{GT_k - FN_k}\\
\frac{\partial UOI_k}{\partial FN_k} = \frac{-(GT_k+FP_k)}{(GT_k - FN_k)^2}
\end{gather}

We can observe that these gradients complement each other. This behaviour is much more desirable in comparison to that of IOU.



\paragraph{Does UOI optimise IOU?}
	Since it is clear that $UOI_k$ has more desirable properties compared to $IOU_k$, it would appear that UOI ($=\sum_k UOI_k$) would perform better as an objective function compared to IOU ($=\sum_k IOU_k$). We provide empirical proof for the validity of this assumption through the plots in figure [number]. The gradients of IOU converge to zero for a large number of false labels which is similar to the behavior of $IOU_k$. A similar parallel can be observed between $UOI$ and $UOI_k$.
	
	
\subsection{Does UOI optimise IOU?}

	Since we have now established that the UOI function has more desirable traits, we have to understand whether there exists a correlation in between the two objectives defined in [eq(1) and eq(6)]. In other words, we have to show that minimisation of UOI leads to the maximisation of IOU.
	
	We argue that there exists a lower bound on the IOU for a fixed UOI. In other words, if we can show that there exists a decreasing function `$f$' such that,
\begin{equation}
\sum IOU_k \ge f(\sum UOI_k)
\end{equation}
then we can say that decreasing value of UOI leads to increasing value of the lower-bound on  IOU. Further, we also have to show that the maximum possible value of IOU(=K) is achievable.


Suppose the decreasing function `$f$' is defined as:
$$f(x)=\frac{1}{x}$$
We have to now show that:
\begin{enumerate}
\item $\sum IOU_k \ge \frac{1}{\sum UOI_k}$
\item There exists a value of UOI for which IOU=K
\end{enumerate}


Assume that $x_k=IOU_k$, we know that
\begin{gather}
0\le x_k \le 1\\
\Rightarrow \frac{1}{x_k} \ge \frac{1}{\sum_k x_k}\\
\Rightarrow \sum_k\frac{1}{x_k} \ge \frac{1}{\sum_k x_k}\\
\Rightarrow \sum_k{x_k} \ge \frac{1}{\sum_k\frac{1}{x_k}}\\
\Rightarrow \sum_k IOU_k \ge \frac{1}{\sum_k UOI_k}
\end{gather}


Hence, the lower-bound of IOU has been shown as a decreasing function of UOI. In the case where each of $UOI_k=1$, clearly, $\sum_{k=1}^K IOU_k=K$. This implies that UOI acts as a good objective function for optimising IOU.






\paragraph{Losses}
We tried two loss functions, the first being cross entropy averaged over each
pixels of of the soft $13 \times 13$ segmentations and the second
being Intersection Over Union. The first is standard, but we'll describe
IOU in more detail.

Let $\hat{p}_{ik}$ denote the probability of class $k$ predicted at pixel $i$
by the last layer of a \segnet and $p_{ik}$ denote the same thing for ground truth.
Expected intersection is given by
\begin{equation} \label{eq:int}
    E[I_k] = \sum_i \hat{p}_{i, k} p_{i, k}^m
\end{equation}
and the expected union is given by
\begin{equation} \label{eq:union}
    E[U_k] = \sum_i \hat{p}_{i, k} + p_{i, k}^m - \hat{p}_{i, k} p_{i, k}^m
\end{equation}
Now we can define IOU loss:
\begin{equation} \label{eq:iou}
    \mathcal{L}(\bm{\hat{p}}, \bm{p}) = \sum_{k} \frac{E[I_{k}(\bm{\hat{p}}, \bm{p})]}{E[U_{k}(\bm{\hat{p}}, \bm{p})]}
\end{equation}
Theoretically, the idea of IOU aligns with semantic segmentation better than
cross-entropy. Notice that
\begin{enumerate}
    \item
    Classes are weighted equally instead contributing to the loss
    in proportion to their pixel count.

    \item
    The loss does not break down over pixels.

    \item
    If equations \ref{eq:int} and \ref{eq:union} are summed over pixels in a
    batch instead of pixels in an image then the loss doesn't even break down
    over examples. Since the PASCAL metric computes
    this corpous wide IOU, it is a closer approximation than optimizing
    an IOU which is computed per-image.
    When the batch size is the size of the dataset the approximation is exact.
\end{enumerate}


==> space_saver.tex <==
% Some illegal space-saving macros
\parskip=3pt
\abovedisplayskip 3.0pt plus2pt minus2pt%
\belowdisplayskip \abovedisplayskip
%\renewcommand{\baselinestretch}{0.98} % VERY powerful and VERY illegal. Use carefully

\newlength{\sectionReduceTop}
\newlength{\sectionReduceBot}
\newlength{\subsectionReduceTop}
\newlength{\subsectionReduceBot}
\newlength{\abstractReduceTop}
\newlength{\abstractReduceBot}
\newlength{\captionReduceTop}
\newlength{\captionReduceBot}
%\newlength{\nameReduceTop}
\newlength{\subsubsectionReduceTop}
\newlength{\subsubsectionReduceBot}

\newlength{\eqnReduceTop}
\newlength{\eqnReduceBot}

\newlength{\horSkip}
\newlength{\verSkip}

\newlength{\figureHeight}
\setlength{\figureHeight}{1.7in}

%\newlength{\figureFraction}
\setlength{\horSkip}{-.09in}
\setlength{\verSkip}{-.1in}
%\setlength{\figureFraction}{.195}


%
\setlength{\subsectionReduceTop}{-0.12in}
\setlength{\subsectionReduceBot}{-0.09in}
\setlength{\sectionReduceTop}{-0.08in}
\setlength{\sectionReduceBot}{-0.10in}
\setlength{\subsubsectionReduceTop}{-0.06in}
\setlength{\subsubsectionReduceBot}{-0.05in}
%
%
%\setlength{\figureHeight}{1.5in}
\setlength{\abstractReduceTop}{-0.05in}
\setlength{\abstractReduceBot}{-0.10in}
%
%

\setlength{\eqnReduceTop}{-0.05in}
\setlength{\eqnReduceBot}{-0.05in}

%\setlength{\nameReduceTop}{-0.05in}


\setlength{\captionReduceTop}{-0.14in}
\setlength{\captionReduceBot}{-0.12in}
%\setlength{\captionReduceBot}{-0.15in}

